The $p$-curvature conjecture for the non-abelian Gauss-Manin connection

Originally conjectured unpublished by Grothendieck, then formulated precisely by Katz, the $p$-curvature conjecture is a local-global principle for algebraic differential equations. It is at present open, though various cases are known. Katz subsequently proved this conjecture in a wide range of cases, for differential equations corresponding to the Gauss-Manin connection on algebraic de Rham cohomology. This dissertation addresses the non-abelian analogue of Katz' theorem, in the sense of Simpson's non-abelian Hodge theory, surveyed by Simpson and later developed in characteristic $p$ by Ogus and Vologodsky. Specifically, there is a canonical non-abelian Gauss-Manin connection on $M_{dR}$, the stack of vector bundles with integrable connection, which is the appropriate definition of non-abelian de Rham cohomology. In this dissertation, I introduce this connection and its $p$-curvature; this requires the generalization of the $p$-curvature conjecture due to Bost, Ekedahl and Shepherd-Barron. Then, I prove that the analogue of the main technical result of Katz' theorem holds for this connection.

==> copyright.tex <==
% ----------------------------------------------------------------

\thispagestyle{empty} 

\vspace*{\fill}

\begin{center}
\copyright \, 2019 -- Max Menzies \\
All rights reserved.
\end{center}

\vspace*{\fill}

\pagebreak

% ----------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

% ----------------------------------------------------------------

==> title.tex <==
% ----------------------------------------------------------------

\thispagestyle{empty}

\vspace*{\fill}

\begin{center}
The $p$-curvature conjecture for the non-abelian Gauss-Manin connection\\
\vspace{0.2in}
A dissertation presented\\
\vspace{0.2in}
by\\
\vspace{0.2in}
Max Menzies\\
\vspace{0.2in}
to\\
\vspace{0.2in}
The Department of Mathematics\\
\vspace{0.2in}
in partial fulfillment of the requirements\\
for the degree of\\
Doctor of Philosophy\\
in the subject of\\
Mathematics\\
\vspace{0.2in}
Harvard University\\
Cambridge, Massachusetts\\
\vspace{0.2in}
April 2019\\
\end{center}

\vspace*{\fill}

\pagebreak

%\maketitle

% ----------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

% ---------------------------------------------------------------- 
